An Ensemble Approach for Automated Theorem Proving Based on Efficient Name Invariant Graph Neural Representations

Using reinforcement learning for automated theorem proving has recently received much attention. Current approaches use representations of logical statements that often rely on the names used in these statements and, as a result, the models are generally not transferable from one domain to another. The size of these representations and whether to include the whole theory or part of it are other important decisions that affect the performance of these approaches as well as their runtime efficiency. In this paper, we present NIAGRA; an ensemble Name InvAriant Graph RepresentAtion. NIAGRA addresses this problem by using 1) improved Graph Neural Networks for learning name-invariant formula representations that is tailored for their unique characteristics and 2) an efficient ensemble approach for automated theorem proving. Our experimental evaluation shows state-of-the-art performance on multiple datasets from different domains with improvements up to 10% compared to the best learning-based approaches. Furthermore, transfer learning experiments show that our approach significantly outperforms other learning-based approaches by up to 28%.

==> sections/challenges.tex <==
\section{Motivation}


==> sections/graph_representation.tex <==
\section{Efficient Name Invariant Graph Representation}

\begin{figure}
\begin{center}
% \includegraphics[width=0.7\columnwidth] {figures/clause_repr_ex.pdf}
\includegraphics[width=0.7\columnwidth]{figures/clause_repr_ex2.pdf}

\caption{DAG representation of the clause $\forall A, B, C .\ p(A) \vee \lnot q(B, f(A)) \vee q(C, f(A))$ where variable labels are replaced with generic tokens to ensure invariance to arbitrary variable renaming}
\label{fig:dag_example}
\end{center}
\end{figure}


\begin{figure*}
\begin{center}
% \includegraphics[width=0.7\columnwidth] {figures/clause_repr_ex.pdf}
\includegraphics[width=2\columnwidth]{figures/shared_names_merged.pdf}

\caption{Example representation of two clauses with (left) and without (right) user-defined names sharing. Information about user-defined names  appears only in the square nodes. }
\label{fig:dag_example}
\end{center}
\end{figure*}

\subsection{The problem and motivation}
Recently, multiple graph representations have been proposed to represent logical formulas as part of machine learning-based proof guidance systems for automated theorem provers ~\cite{TRAIL, DeepMind} . A logical formula is first converted into a directed acyclic graph (DAG). Then, different graph neural networks can be applied to the resulting DAG to produce a dense vector representation of the input logical formula. In prior work, each logical formula is converted into a separated graph disconnected from the graphs representing other formulas as shown in Figure~\ref{fig:dag_example} and ~\ref{fig:disconnected_graph}. The embeddings of those isolated graphs are then independently computed using graph neural networks. This simple approach is very efficient in terms of run-time performance and reduced overhead for two main reasons:
\begin{itemize}
    \item  it enables the parallel computation of the embeddings of formulas, and
    \item it also enables the reuse of those embeddings within a proof attempt since the graph used to compute  embeddings of a formula is unchanged throughout the reasoning process. 
\end{itemize}    
However, in general, this simple approach is not faithful to the semantics of logical formulas.  The meaning of a clause originating from the initial set of axioms, the negation of the conjecture or a derived fact generated during the reasoning process is, in general, a function of all other clauses already processed or available to be processed by the reasoner. 

Ideally, in order to preserve the connections and inter-dependencies between clauses, all clauses should be represented in a single connected directed acyclic graph rooted at a conjunction node as shown in Figure~\ref{fig:connected_graph}.  Unfortunately, such graph constantly involves during the reasoning process as new clauses are generated and added to the graph. The embeddings of clauses change at each reasoning step and need to be constantly recomputed and updated leading to a significant and unacceptable overhead. 

Independent clause embedding approaches such as \cite{DeepMind} recover some of the dependencies between clauses by using the shared user defined names of predicates, functions and constants as part of the embedding of independent clause graph. Unfortunately, this yields to a name sensitive representation, which might work fine if the same vocabulary is used consistently within a given dataset. However, it is likely to struggle to generalize to either a dataset with a completely different vocabulary or a dataset with a vocabulary that overlaps with the training vocabulary, but in which the common names have a completely different meaning (e.g., a functions f and g in the training dataset have been swapped in the test dataset). In fact, predicate, function and constant names are irrelevant artifacts since the meaning of a given logical theory is unchanged after consistently renaming predicates, functions and constants. Including them explicitly, in clause representations, could induce learning of spurious correlations between those irrelevant artifacts and, thus, hinder generalization.  

To avoid name sensitive representations, inspired from recent work on preserving properties such as invariance to predicate, constant, and function names, and variable quantification order  {\color{red}{CITE 62, 71, 42, 45 from TRAIL journal paper}}, \cite{TRAIL} does not rely on user defined predicate, function, and constant names. It produces independent graph representations similar to Figure~\ref{fig:dag_example}, and,  the initial embedding of a node during the GNN computation is only a function of its type (i.e, in Figure ~\ref{fig:dag_example}, the color of the node and its shape - not the label of the node). Unfortunately, this solution has two shortcomings. First, the initial embedding does not preserve the individuality of each symbol (e.g., all square name nodes have the same initial embedding). Second, there is very limited information exchange between disconnected clause graph. Within a single clause graph, all applications of the same function or predicate  (e.g., the two blue nodes labeled q in Figure~\ref{fig:dag_example}) have a direct link to the same user defined name node (e.g., the square node label "q").  Unfortunately, as shown in Figure~\ref{fig:disconnected_graph}, these square user defined name nodes are not connected or shared across clause graphs. As a result, there is little information shared between the two square nodes labeled "q" in  Figure~\ref{fig:disconnected_graph}. They only share the same initial embedding, which is not very informative as it is also shared by all other square nodes (including those labeled "f" and "p").

\subsection{Our solution}

\subsubsection{Three key insights} Our proposed solution is based on the following three key observations:
\begin{itemize}
    \item  In the clausal normal form, after an equivalence preserving  variable renaming, the ideal graph connecting all clauses (from the initial axioms, the negated conjecture, and derived clauses) is such that the only shared nodes across clauses are squared nodes representing names of constants, functions, and predicates as shown in Figure~\ref{fig:connected_graph}. In fact, since the universal quantifier distributes over conjunction, in the clausal conjunctive normal form, we can push the top level universal quantifiers to inside each clause and then safely rename variables within each clause in such a way that two distinct clauses do not have any common variables. Thus, the only shared symbols between clauses are constants, functions and predicate names (including skolem constants and functions introduced during the normalization process to get rid of existentially quantified variables) 
    \item All those user defined and skolem names of constants, functions, and predicates are already present in the original normalized theory\footnote{except for some E inference strategies that can generate a relatively small brand new predicates during reasoning.}
    \item The meaning of all those constant, function and predicate names is fully specified by the set of initial axioms and the conjecture. 
\end{itemize}
Based on those three observations, our proposed solution is the following two-phase approach:
\begin{enumerate}
    \item  In the first phase, before the start of the reasoning process, we learn, from the fully connected graph of the normalized theory and the negated conjecture, the embeddings of the vocabulary of predicates, functions and constants. This enables us to learn meaningful embedding of non-logical symbols in a way that is name invariant and dependent only on the input theory. 

    \item In the second phase, at each step of the reasoning, we use those embeddings as the initial embeddings of name nodes (i.e., square nodes in Figure~\ref{fig:disconnected_graph}) in the independent graph of each new clause so that, across all independent graphs in Figure~\ref{fig:disconnected_graph}, name nodes with different labels receive different initial embeddings while those with the same label start with the same initial embeddings. In doing so, we address the two key issues of lack of name node individuality and limited information sharing across independent clause graphs.
\end{enumerate}
Concretely, in the first phase, we build the fully connected graph $G_0$ of the normalized theory and the negated conjecture such as illustrated in Figure~\ref{fig:connected_graph}.  This fully connected graph is only computed once before performing any inference step, thus limiting the overhead. Using a graph neural network such as StageGCN presented in ~\ref{TRAIL}, we then compute an embedding of all nodes in the connected graph $G_0$. In particular, at the end of this phase, we obtain distinguished embeddings for each constant, function, and predicate name node (i.e., square nodes in Figure~\ref{fig:connected_graph} ), which are later used during reasoning steps as the initial embeddings of corresponding name nodes in independent graphs representing new clauses. 


